Link Prediction and the Role of Stronger Ties in Networks of Face-to-Face Proximity

Understanding the structures why links are formed is an important and prominent research topic. In this paper, we therefore consider the link prediction problem in face-to-face contact networks, and analyze the predictability of new and recurring links. Furthermore, we study additional influence factors, and the role of stronger ties in these networks. Specifically, we compare neighborhood-based and path-based network proximity measures in a threshold-based analysis for capturing temporal dynamics. The results and insights of the analysis are a first step onto predictability applications for human contact networks, for example, for improving recommendations.

==> acknowledgements.tex <==
\section*{Acknowledgements}
This work has been supported by the VENUS research cluster at the interdisciplinary Research Center
  for Information System Design (ITeG) at Kassel University.
%
We utilized active RFID technology which was developed within the SocioPatterns project, whose generous support we kindly acknowledge. 
Our particular thanks go the SocioPatterns team, especially to Ciro Cattuto, who enabled access to the Sociopatterns technology, 
and who supported us with valuable information concerning the setup of the RFID technology.

==> styles.tex <==
\usepackage[utf8]{inputenc}
\usepackage{times}
\usepackage{helvet}
\usepackage{courier}

\usepackage{flafter}
\usepackage{graphicx}
\graphicspath{{figs/}}

\usepackage[utf8]{inputenc}   % option depends of your computer platform
\usepackage[german,american]{babel}
\usepackage[T1]{fontenc}
\fontfamily{ptm}\selectfont

\usepackage{longtable}
\usepackage{float}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amscd}
%\usepackage{amsthm}
\usepackage{bbm}

\usepackage{mathrsfs}
\usepackage{wrapfig}
\usepackage{paralist}
\usepackage{url}
\usepackage{xspace}



